Gaiotto Duality for the Twisted A_{2N-1} Series

We study 4D N=2 superconformal theories that arise from the compactification of 6D N=(2,0) theories of type A_{2N-1} on a Riemann surface C, in the presence of punctures twisted by a Z_2 outer automorphism. We describe how to do a complete classification of these SCFTs in terms of three-punctured spheres and cylinders, which we do explicitly for A_3, and provide tables of properties of twisted defects up through A_9. We find atypical degenerations of Riemann surfaces that do not lead to weakly-coupled gauge groups, but to a gauge coupling pinned at a point in the interior of moduli space. As applications, we study: i) 6D representations of 4D superconformal quivers in the shape of an affine/non-affine D_n Dynkin diagram, ii) S-duality of SU(4) and Sp(2) gauge theories with various combinations of fundamental and antisymmetric matter, and iii) realizations of all rank-one SCFTs predicted by Argyres and Wittig.

==> fullstar.tikz.tex <==



\begin{tikzpicture}[y=0.80pt, x=0.8pt,yscale=-1, inner sep=0pt, outer sep=0pt]
  \path[draw=black,fill=black,line width=1.600pt] (7.2500,2.0000) --
    (8.3750,5.1875) -- (11.7500,5.1875) -- (9.1250,7.2500) -- (10.0625,10.4375) --
    (7.2500,8.5625) -- (4.4375,10.4375) -- (5.3750,7.2500) -- (2.7500,5.1875) --
    (6.1250,5.1875) -- cycle;

\end{tikzpicture}

